Software Product Line for Metaverse: Preliminary Results

The Metaverse is a network of eXtended Reality applications (XR apps) connected to each other, over the Internet infrastructure, allowing network users, systems, and devices to access them. It is very challenging to implement solutions for XR apps, due to the combination of complex concerns that should be addressed: multiple users with non-traditional input and output devices, different hardware platforms that should be addressed, forceful interactive rates, and experimental interaction techniques, among other issues. Therefore, this work aims to present a Software Product Line (SPL)-based approach to support the development of Web XR apps. More specifically, we define a features model that represents similarities and variables (domain analysis); we defined a core composed of generic and reusable software artifacts (domain project); and we developed an interface to support the instantiation of a Web XR app family, named MetaSee Features Model Editor (domain implementation). This approach integrates with a component of the MetaSEE architecture (Metaverse for Software Engineering Education). A preliminary assessment found that Features Model has conceptual consistency from the point of view of the complexity of Web XR Apps multimodal interaction. As future work, features model and artifacts will be increased with improvements and an evaluation with a significant number of participants will be made.

==> Sections/Approach_2.tex <==
\section{Approach} \label{sec:approach}

% introduction to the section

\subsection{Context} \label{sec:context-approach}
MetaSEE (Metaverse for Software Engineering Education) é uma abordagem para integrar mundos virtuais de SEE e tem como objetivo preencher uma lacuna identificada por meio de uma revisão sistemática da literatura  \cite{fernandes_systematic_2022}. A partir dos achados da revisão, a arquitetura do MetaSEE foi projetada baseada em três requisitos fundamentais: SEE, feasibility factors, and components and technologies. 

SEE requirements estabelecem as características que a arquitetura deve atender para o domínio. Elas foram baseadas nas limitações dos mundos virtuais encontradas pela revisão. Portanto, a arquitetura deve: 
cover any SE topic; support the analysis of learning performance data; implement new forms of visualization and interaction; facilitate development for the Metaverse; 
perform analyzes using biometric data; and ensure data interoperability.

The Metaverse needs four factors to make it viable \cite{dionisio_3d_2013}. Therefore, the architecture must consider the following feasibility factors:
\textit{realism} enables users to feel fully immersed in an alternative universe;
\textit{ubiquity} establishes access to the system via all existing digital devices and maintains the user's virtual identity throughout transitions within the system;
\textit{interoperability} is a connected collection of information, format, and data standards, most of which focus on the transfer of 3D models across virtual worlds, in addition to involving communication protocol, identity, and currency standards; and \textit{scalability} allows concurrent efficient use of the system by massive numbers of users.

Components and technologies requirements estabelecem os principais aspectos de o Metaverso identificados através de uma análise comparativa de pesquisas recentes \cite{fernandes_systematic_2022}: authoring tools; devices; economy; infrastructure; interaction; physical world; security; storage; technology; and virtual world.


Como resultado, a arquitetura do MetaSEE estabelece os principais elementos para viabilizar o Metaverso especificamente entre mundos virtuais de SEE. Fig. \ref{fig:metasee-overview} presents the design of the MetaSEE e seus principais elementos agrupados em 5 camadas.

\textit{Physical Layer} corresponds to the main entities external to the Metaverse and that belong to the physical and real world. \textit{Virtual Layer} establishes the main components of the "virtualization" of physical layer elements. In \textit{Metaverse Engine Layer} establishes the general technologies, as well as economics and security of the Metaverse. \textit{MetaSEE Layer} is the main contribution to support SEE through the Metaverse. According to the established fundamental requirements, it was defined development tools, integrantion tools, and Learning Analytics (LA) as the components of this layer. Finally, \textit{Infrastructure Layer} deals with network and decentralization aspects of the Metaverse. 

\begin{figure}[!h]
    \centering
    \includegraphics[scale=.5]{Figures/MetaSEEOverview.png}
    \caption{MetaSEE architecture overview \cite{fernandes_systematic_2022}}
    \label{fig:metasee-overview}
\end{figure}

In fact, MetaSEE is an overview of essential elements in order to specifically enable a Metaverse for SEE. Although its structure seems to serve any area with educational purposes, its main objective is to adopt a strategy of integrating XR apps for SEE and facilitating its adoption by the SEE community.

Therefore, as shown in Fig. \ref{fig:metasee-platform}, MetaSEE platform is an XR app that should make a link between users (e.g., students and teachers) and other XR apps for SEE. From the platform, the user will be able to choose which virtual world to ``enter" or ``exit", according to the approach and topic of SE addressed, in addition to ensuring data traceability for future analysis and improvement of teaching experiences. Additionally, developers will have access to development and integration tools serving as support in the reuse of features by XR apps, as well as in the development of new applications.

\begin{figure}[!h]
    \centering
    \includegraphics[scale=.3]{Figures/MetaSEEplatform.png}
    \caption{MetaSEE platform overview}
    \label{fig:metasee-platform}
\end{figure}

\section{MetaSEE Features Model} \label{sec:features-model}

MetaSEE Features Model foi desenvolvida com as seguintes etapas:
(i) análise de domínio;
(ii) definição de um modelo de aplicativo; e 
(iii) desenvolvimento de uma interface para instanciação dos aplicativos.

A análise de domínio define o escopo da SPL.
O modelo de aplicativo descreve os principais elementos de maneira genérica.
A interface fornece parâmetros baseado no modelo para gerar o esqueleto de código a serem reutilizados pelos Web XR apps.

\subsection{Análise de Domínio}

A análise de domínio foi realizada sobre Web XR apps existentes para a definição do escopo da SPL desenvolvida.

Essa etapa resultou, basicamente, em três produtos:
(i) uma lista de requisitos gerais para Web XR apps;
(ii) a lista das funcionalidades para o usuário final, classificadas de acordo com a presença nos aplicativos existentes e possibilidade de reúso; e
(iii) a modelagem das características da SPL, baseadas nesses requisitos e funcionalidades, representada por um diagrama de características.

Os requisitos gerais dos Web XR apps existentes são:
(i) funcionar em navegadores Web; 
(ii) permitir o uso de dispositivos tradicionais (e.g., desktop e smartphone) e não tradicionais (e.g., XR headset e dataglove);
(iii) utilizar os sentidos humanos para o engajamento de experiências imersivas; e
(iv) permitir várias formas de interação.

Esses requisitos, em conjunto com as funcionalidades pontuais, foram classificados com relação à presença nos aplicativos. Uma funcionalidade comum é aquela que está ou poderia estar presente em mais de um membro da família, enquanto que uma funcionalidade específica está presente em apenas um aplicativo e não pode ser incluída nos demais.

Esse mapeamento resultou na definição das características da SPL, apresentadas
no diagrama da Fig. \ref{fig:features-model}.

% ARRUMAR
Existem basicamente três tipos de características:
(i) as obrigatórias, presentes em todos os aplicativos%, identificadas com traços simples na figura;
(ii) as alternativas, que cada aplicativo possui apenas uma das possibilidades, %identificadas com um arco sobre as opções; e
(iii) as opcionais, em que um aplicativo pode ou não possuir%, identificadas por um círculo ao fim do traço.

\begin{figure}
    \centering
    \includegraphics{}
    \caption{Features model for Web XR apps}
    \label{fig:features-model}
\end{figure}

No diagrama, um Web XR app é descrito pelas características obrigatórias Platform, Multimodal Interfaces, XR Modality, Devices, Browser, Avatar, and Virtual World.

Platform é um ponto de variação que estabelece as variantes do tipo de dispositivo que o aplicativo será executado. Wearable representa os dispositivos imersivos (não tradicionais), tais como XR headset, haptic devices, motion sensors, etc. Desktop and Mobile representam os dispositivos comuns de interação entre o usuário e computador.

Multimodal Interfaces é um ponto de variação que estabelece quais as modalidades (i.e., human senses) que podem estar presentes nos aplicativos a fim de possibilitar o engajamento das experiências imersivas. A modelagem desta variabilidade é baseada na taxonomia de modalidades de interação para XR \cite{augstein_human-centered_2019}.
Direct processing works directly between a computer and the brain or muscles. Indirect processing refers to the multi-stage process where an output stimulus is perceived by a human receptor and then the information is delivered via electrical signals for further processing to the brain. The flow is similar for input stimulus from a human via sensors to the computer.

Nós baseamos no Milgram’s Reality-Virtuality (RV) continuum \cite{milgram_augmented_1995} para definir as variantes da XR Modality. Virtual Reality considera somente objetos virtuais para compor o mundo virtual do aplicativo e Mixed Reality combina elementos do mundo real e objetos virtuais para compor o mundo virtual. 

Devices corresponde aos dispositivos que serão utilizados tanto para interação quanto para feedback (e.g., Meta Quest, HTV Vive, Hololens); Browser é o navegador web que terá compatibilidade com o aplicativo, Avatar é a representação do usuário, and Virtual World é o espaço virtual no qual o usuário é inserido para interagir com os objetos virtuais.

A única característica opcional da modelagem é Interaction Events. Ela estabelece os eventos de interação para cada tipo de dispositivo. Por exemplo, a implementação do evento ``click" considerando a execução de um aplicativo no desktop é diferente em um XR headset. No desktop este evento é disparado através do botão do mouse, porém no XR headset pode ser através de qualquer botão do seu controlador. Essa caraterística é opcional, pois um aplicativo pode somente exibir objetos virtuais sem necessitar qualquer tipo de interação e/ou feedback.
%No diagrama, uma iMA é descrito pelas características obrigatórias: todas as de Comunicação, de Configuração e de Gerenciamento de Atividades, apenas uma das Operações de Domínio, que representam as funcionalidades específicas do domínio de cada iMA (geometria, combinatória, etc.), e quais opcionais possui das categorias Funcionalidades sobre Atividades e Funcionalidades sobre Operações de Domínio.

\subsection{Modelo de Sistema}
A partir da identificação das características, uma arquitetura de sistema foi criada para definir o funcionamento interno de um Web XR app de maneira independente das funcionalidades específicas de cada aplicativo.

Essa tarefa intermediária teve objetivo de permitir que o núcleo da SPL fosse independente de domínio, ou seja, para que o núcleo não estivesse preso às características de algum Web XR app específico.

O resultado foi a produção de uma arquitetura (see Fig. \ref{fig:generic-arch}) que é composta por quatro componentes:
(i) Features: representa as features que irão compor a instância do aplicativo;
(ii) WebXR Framework: define o framework que atuará como interface entre o código HTML5 e dispositivo;
(iii) XR Component: importa os componentes necessários para a instanciação das feautures conforme o WebXR framework escolhido; e
(iv) Template Generator: provê mecanismos para a geração de esqueleto de código baseado nas opções escolhidas anteriormente.

\begin{figure}
    \centering
    \includegraphics{}
    \caption{Generic architecture of SPL for Web XR app}
    \label{fig:generic-arch}
\end{figure}



% (i) estrutural, que oferece a base e as funcionalidades comuns;
% (ii) atividades, que define as atividades para os alunos, autoria por professores e correção automática;
% (iii) domínio, que modela genericamente os objetos e as operações de domínio; e (iv) expansões, que modela genericamente as funcionalidades sobre atividades ou operações de domínio [Dalmon et al. 2012b].


\subsection{Interface de Instanciação}

Uma interface de instanciação de Web XR apps foi escolhida como forma de implementação do núcleo da SPL por atender aos requisitos e características desejadas, que incluem promover reúso de código, reúso de arquitetura e não exigir conhecimentos avançados de programação para utilização por outros desenvolvedores [Guerra 2011]. %Além de ser possível criar um método de desenvolvimento a partir dos pontos flexíveis do arcabouço.

Interface de instanciação para desenvolvimento de Web XR apps foi derivado diretamente do modelo de sistema descrito acima. O diagrama de componentes da versão atual do arcabouço é mostrado na Figura 2. %Os componentes com nome em negrito são parte do núcleo comum e fornecem as funcionalidades obrigatórias, aqueles em itálico e sublinhado têm o papel de implementar as operações de domínio, específicas para cada iMA, e os com nome em fonte monoespaçada representam as funcionalidades opcionais.





% O objetivo deste trabalho é apresentar a implementação do protótipo MetaSEE Features Model, no qual integra o componente \textit{Development Tools} da arquitetura MetaSEE (see Fig. \ref{fig:metasee-overview}. This component provides a set of tools to facilitate the development of XR apps for SEE.

% MetaSEE Features Model é uma ferramenta que permite a instanciação de aplicações a partir de um modelo que define características opcionais, mandatórias, variáveis e invariáveis de Web XR apps. 















==> Sections/Discussion.tex <==
\section{Discussion} \label{sec:disucssion}

==> Sections/ProofOfConcept.tex <==
\section{Proof of Concept} \label{sec:proofofconcept}



==> TODO.tex <==
TODO

- strategy paper: creating a features model and to validate it with academic/expert persons.

CHECK

- to verify abbreviations:
    SE - Software Engineering (SE)
    SEE - Software Engineering Education (SEE)
    XR - eXtended Reality (XR)
    XR apps - eXtended Reality Applications (XR apps)
    DE - Domain Engineering (DE)
    AE - Application Engineering (AE)
    SPL - Software Product Line (SPL)
